GIGA-Lens: Fast Bayesian Inference for Strong Gravitational Lens Modeling

We present GIGA-Lens: a gradient-informed, GPU-accelerated Bayesian framework for modeling strong gravitational lensing systems, implemented in TensorFlow and JAX. The three components, optimization using multi-start gradient descent, posterior covariance estimation with variational inference, and sampling via Hamiltonian Monte Carlo, all take advantage of gradient information through automatic differentiation and massive parallelization on graphics processing units (GPUs). We test our pipeline on a large set of simulated systems and demonstrate in detail its high level of performance. The average time to model a single system on four Nvidia A100 GPUs is 105 seconds. The robustness, speed, and scalability offered by this framework make it possible to model the large number of strong lenses found in current surveys and present a very promising prospect for the modeling of $\mathcal{O}(10^5)$ lensing systems expected to be discovered in the era of the Vera C. Rubin Observatory, Euclid, and the Nancy Grace Roman Space Telescope.

==> figures/summary.tex <==
% \begin{deluxetable}{l p{3.5cm} p{6.25cm} c c}
% \tablecaption{Summary of the modeling pipeline\label{tab:pipeline}. The typical execution time for running each step on the V100 GPU and 4 A100 GPUs are reported.}
% \tablehead{
% \colhead{Step} & \colhead{Output} & \colhead{Hyperparameters} & \colhead{Time (V100)} & \colhead{Time (A100 $\times$ 4)}}
% \startdata
% 1. MAP & An estimate of the posterior mode $\tilde{\Theta}^*_{global}$. & 
% Number of starts $n_{MAP}=300$, number of iterations $k=300$, learning rate $\alpha=10^{-2}$ to $\alpha=10^{-3}$ over $k$ iterations 
% & 2 minutes & 17 seconds \\
% 2. VI & An estimate of the posterior mean $\tilde{\mu}^*$ and covariance $\tilde{\Sigma}^*$. & Initial guess $\tilde{\mu}$, $\tilde{\Sigma}$, number of samples for estimating the ELBO $n_{VI}=500$, number of iterations $k=1500$, learning rate that is annealed from $\alpha=10^{-6}$ to $\alpha=10^{-3}$ over 200 iterations.  & 3 minutes  & 52 seconds \\
% 3. HMC & Samples drawn from the posterior $p(\Theta \mid \mathcal{I}_{obs})$. & Number of walkers $n_{HMC}=50$, number of burn-in iterations $n_{burn}=250$, number of sampling iterations $n_{samples}=750$, initial step size $\epsilon=0.3$, initial number of leapfrog steps $L=3$. We use the Tensorflow Probability default hyperparameters for the adaptation of $\epsilon$ and $L$ (e.g., the target acceptance probability for $\epsilon$-adaptation is 0.75). & 4 minutes & 36 seconds \\
% \textbf{Total} & & & \textbf{9 minutes} & \textbf{105 seconds}
% \enddata
% \end{deluxetable}
\begin{deluxetable}{c m{3.5cm} r l c}
\tablecaption{Summary of the modeling pipeline\label{tab:pipeline}}
\tablehead{
\colhead{\textbf{Step}} & \colhead{\textbf{Output}} & \multicolumn2c{\textbf{Hyperparameters}} & \colhead{\textbf{Time (V100/A100 $\mathbf{\times}$ 4)}}}
\startdata
\arrayrulecolor{gray}
& \multirow{3}{=}{An estimate of the posterior mode $\tilde{\Theta}^*_{global}$.} & Number of iterations $K_{MAP}$: & 300 & \\
1. MAP & & Number of samples $n_{MAP}$: & 300 & 2 min. / 17 sec. \\
& & Learning rate $\alpha$: & $10^{-2} \overset{\text{lin,300}}{\longrightarrow} 10^{-3}$ & \\
\hline
%
& \multirow{5}{=}{An estimate of the posterior mean $\tilde{\mu}^*$ and covariance $\tilde{\Sigma}^*$.} & Number of iterations $K_{VI}$: & 1000 & \\
& & Number of VI samples $n_{VI}$: & 500 & \\
2. SVI & & Initial mean $\tilde{\mu}^{(1)}$ & $\tilde{\Theta}^*_{global}$ & 3 min. / 52 sec. \\
& & Initial covariance $\tilde{\Sigma}^{(1)}$: & $10^{-3} \mathbb{I}$ & \\
& & Learning rate $\alpha$: & $0 \overset{\text{quad,500}}{\longrightarrow} 10^{-3}$ & \\
\hline
%
& \multirow{5}{=}{Samples drawn from the posterior $p(\Theta \mid \mathcal{I}_{obs})$} & Burn-in steps $n_{burn}$: & $250$ & \\
& & Sampling steps $n_{sample}$: & 750 & \\ 
3. HMC & & Number of chains $n_{HMC}$: & 50 & 4 min. / 36 sec. \\
& & Initial step size $\epsilon$: & 0.3 & \\
& & Initial leapfrog steps $L$: & 5 & \\
\hline\arrayrulecolor{black}
%
\textbf{Total} & & & & \textbf{9 min.} / \textbf{105 sec.}
\enddata
\tablecomments{We adopt the notation $\alpha_1 \overset{p,k}{\longrightarrow} \alpha_2$ to indicate a learning rate that changes from $\alpha_1$ to $\alpha_2$ over $k$ iterations with a polynomial schedule $p$. The rightmost column indicates typical execution times for each modeling step on the V100 GPU and four A100 GPUs.}
\end{deluxetable}

